Blocked Clusterwise Regression

A recent literature in econometrics models unobserved cross-sectional heterogeneity in panel data by assigning each cross-sectional unit a one-dimensional, discrete latent type. Such models have been shown to allow estimation and inference by regression clustering methods. This paper is motivated by the finding that the clustered heterogeneity models studied in this literature can be badly misspecified, even when the panel has significant discrete cross-sectional structure. To address this issue, we generalize previous approaches to discrete unobserved heterogeneity by allowing each unit to have multiple, imperfectly-correlated latent variables that describe its response-type to different covariates. We give inference results for a k-means style estimator of our model and develop information criteria to jointly select the number clusters for each latent variable. Monte Carlo simulations confirm our theoretical results and give intuition about the finite-sample performance of estimation and model selection. We also contribute to the theory of clustering with an over-specified number of clusters and derive new convergence rates for this setting. Our results suggest that over-fitting can be severe in k-means style estimators when the number of clusters is over-specified.

==> blocked multiple regression - arxiv/figure_convergence_angle.tex <==
\begin{figure}
\centering
\caption{Algorithm Convergence and Cluster Separation}
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{comp1_param.png}
    \caption{$r_{\theta}(s)$}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{comp1_q.png}
    \caption{$r_{Q}(s)$}
  \end{subfigure}
  \label{figure:computation:convergence_angle}
\end{figure}


==> blocked multiple regression - arxiv/figure_convergence_clusters.tex <==
\begin{figure}
\centering
\caption{Algorithm Convergence and Number of Clusters $k = k_1 + k_2$}
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{comp3_param.png}
    \caption{$r_{\theta}(s)$}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{comp3_q.png}
    \caption{$r_{Q}(s)$}
  \end{subfigure}
  \label{figure:computation:convergence_cluster}
\end{figure}

==> blocked multiple regression - arxiv/figure_convergence_nt.tex <==
\begin{figure}
\centering
\caption{Algorithm Convergence and $(N, T)$}
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{comp2_param_n.png}
    \caption{$r_{\theta}(s)$}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{comp2_param_t.png}
    \caption{$r_{\theta}(s)$}
  \end{subfigure}
  \label{figure:computation:convergence_nt}
\end{figure}


==> blocked multiple regression - arxiv/old_text.tex <==
%%% OLD COMPUTATIONAL SECTION ON FULL AND PARTIAL UPDATES

The current implementation of our algorithm performs coordinate ascent on $\theta$ by updating one matrix $\theta_{\ell}$ at a time, as described below in the partial update case. 
An alternative is to solve the full update for all of the blocks $1 \leq \ell \leq \numgroups$ simultaneously, though this is potentially much slower computationally. 
Both alternatives are described below. \\

\textbf{Full Parameter Update} \\

In step (3) of our algorithm,we can perform a full parameter update, setting $\theta^{t + 1} = \argmin_{\theta \in \Theta} \samplerisk(\theta, \gamma^{t + 1})$
To describe the full update, we define $\indsubcluster = \{i: \gamma_{\ell}(i) = a\}$, where $a \in [k_{\ell}]$.
Recall that $\theta = \{\theta_1, \dots, \theta_{\ell}\}$, the collection of parameters for each block, and we can view $\theta_{\ell}$ as a matrix $\theta_{\ell} \in \mathbb{R}^{d_{\ell} \times k_{\ell}}$ that collects the parameters for each cluster in the block in the columns of $\theta_{\ell}$.
Then setting $\nabla_{\thetasuba} \samplerisk(\theta, \gamma) = 0$ gives

\begin{align*}
\sum_{i \in \indsubcluster} y_i \xell &= \sum_{\ellt} \sum_{i \in \indsubcluster} \sum_{t} \xell \xellp \theta_{\ellt}(c_i) = \sum_{\ellt} \sum_{i \in \indsubcluster} \sum_{t} \sum_{b = 1}^{k_{\ellt}} \mathds{1}(\cilt = b) \xell \xellp \theta_{\ellt}(c_i) \\
&= \sum_{\ellt} \sum_{b=1}^{k_{\ellt}} \left (\sum_{t, i \in \indsubcluster} \mathds{1}(\cilt = b) \xell \xellp \right ) \theta_{\ellt b} \equiv \sum_{\ellt} \sum_{b=1}^{k_{\ellt}} M_{\ell a, \ellt b} \theta_{\ellt b}
\end{align*}

Define $\vect(\theta) = (\vect(\theta_1), \dots, \vect(\theta_{\numgroups}))$ and $v_{\ell a} = \sum_{i \in \indsubcluster} y_i \xell$, then $\argmin_{\theta \in \Theta} \samplerisk(\theta, \gamma)$ is given by the solution to 

\begin{equation} \label{full_update}
v = M \vect(\theta)
\end{equation}

Here indices of the form $M_{\ell a, \ellt b}$ are block indices, e.g. giving the indices corresponding to the $a^{th}$ cluster of the $\ell^{th}$ block. 
Letting $d_{max} \equiv \max_{\ell} d_{\ell}$, then the time complexity of the algorithm that solves the equation in \ref{full_update} is $\bigo \left (n d_{max}^2 + \left ( \sum_{\ell} k_{\ell} d_{\ell} \right )^3 \right)$ (assuming cubic time to solve the linear equation).
Note that many of the $M_{\ell a, \ellt b }$ sub-matrices may be zero, so it's possible that a sparse solver may do better. \\

\textbf{Partial Parameter Update} \\

Another option is to update $\theta = (\theta_1, \dots \theta_{\numgroups})$ sequentially, e.g. letting 

\[
\theta_{\ell}^{t + 1} = \argmin_{\theta \in \Theta_{\ell}} L_{N, T}(\theta^{t + 1}_{1:\ell-1}, \theta_{\ell}, \theta^t_{\ell + 1:\numgroups}, \gamma^{t + 1})
\]

for each $1 \leq \ell \leq \numgroups$.
By additive separability of $\samplerisk$ in $\theta_{\ell a}$ over $a \in [k_{\ell}]$, this is equivalent to solving 

\[
\argmin_{\thetasuba \in \mathbb{R}^{d_{\ell}}} \sum_{t, i \in \indsubcluster} (y_{it} - \xell' \thetasuba - f(x_{it}, \theta_{- \ell}))^2
\]

This can be solved by computing the panel regression of $y_{it} - f(x_{it}, \theta_{- \ell})$ on $\xell$ over the subset $\indsubcluster$.
Repeating this for each $1 \leq \ell \leq \numgroups$ and $a \in [k_{\ell}]$ has time complexity $\bigo \left (n d_{max}^2 + \sum_{\ell} k_{\ell} d_{\ell}^3 \right )$, potentially significantly better than (the naive implementation of) the full update above. \\

\textbf{Initialization} \\

In our simulations, we let initialize cluster assignments by setting $\cil^1 \sim \{1, \dots, k_{\ell}\}$ uniformly, and independently over $i, \ell$.
We take $\thetasuba \sim N(0, 1)$, independently over $\ell, a$. 
There are some other potential initialization schemes that may lead to quicker convergence in practice. 


%%% Previous ``throw away extra clusters'' approach to proving rates / consistency for the over-specified estimator

\subsection{Old Approaches [Not Currently Used]}

% WORKING PROOF
In what follows, we outline an attack on (i). 
We start by describing the sense in which $\thetak$ is consistent for $\theta^0$ when $k \geq k^0$. 
With $\qtilde$ defined as in our consistency proof in equation \ref{equation:qtilde_def}, we have 
\begin{align*}
\qtilde(\thetak, \gammak) &= \wh{Q}(\thetak, \gammak) + [\qtilde(\thetak, \gammak) - \wh{Q}(\thetak, \gammak)] \leq \wh{Q}(\thetak, \gammak) + \sup_{\theta \in \Theta^k, \gamma \in \Gamma^k} \left [(\qtilde - \wh{Q})(\thetak, \gammak) \right ]\\
&= \wh{Q}(\thetak, \gammak) + o_P(1) \leq \wh{Q}(\theta^0, \gamma^0) + o_P(1) = \qtilde(\theta^0, \gamma^0) + o_P(1) 
\end{align*}

% note - can make cmpt assumption more explicit for k not k^0
The third expression  
Note that we now sup over $(\Theta^k, \Gamma^k)$, but the second inequality still holds as long as $\text{Im}(\theta^k \circ \gamma^k)$ is compact.  
The second inequality still holds because $k \geq k^0 \implies$ $(\theta^0, \gamma^0)$ is in the parameter space of the misspecified estimator.\footnote{Specifically, there exist $\theta^k \in \Theta^k$ and $\gamma^k \in \Gamma^k$ such that the $N \times p$ matrix with i^{th} row $\theta^0(\gamma^0(i)) = \theta^k(\gamma^k(i))$ for all $i \in [N]$}
This shows that $0 \leq \qtilde(\thetak, \gammak) - \qtilde(\theta^0, \gamma^0) \leq o_P(1)$. 
Then our proof of part (ii) of the lemma shows
\begin{align*}
o_p(1) &\geq \qtilde(\thetak, \gammak) - \qtilde(\theta^0, \gamma^0) = \frac{1}{NT}\sum_{i, t} (x_{it}'(\theta^0(c_i^0) - \wh{\theta}^k(\cest^k))^2 \\
&\geq \delta \sum_{c' \in \mathcal{C}^{k_0}} \min_{x \in \mathcal{C}^k} \|\wh{\theta}^k(x) - \theta^0(c')\|^2 - o_p(1) \\
&\implies \min_{x \in \mathcal{C}^k} \|\wh{\theta}^k(x) - \theta^0(c)\|^2 = o_p(1) \quad \forall c \in \clusterspace^{k_0}
\end{align*}

using compactness in the second inequality. 
Since the square norm above is additively separable in the norms of each block of the covariate vector, for any $c, c' \in \clusterspace^{k_0}$ with $c_{\ell} = c'_{\ell}$, we must have $(\argmin_{x \in \clusterspace^k} \|\wh{\theta}^k(x) - \theta^0(c)\|^2)_{\ell} = (\argmin_{x \in \clusterspace^k} \|\wh{\theta}^k(x) - \theta^0(c')\|^2)_{\ell}$. 
This shows that setting $\sigma_{\ell}(a) = (\argmin_{x \in \clusterspace^k} \|\wh{\theta}^k(x) - \theta^0(c)\|^2)_{\ell}$ for any $c \in \clusterspace^{k_0}$ with $c_{\ell} = a$ is well-defined. 
As in the well-specified case, this relationship is 1-1 w.h.p. as $N, T \to \infty$ by well-separation of the true clusters in assumption \ref{consistency:separation}, so we relabel $\thetak_{\ell a} \equiv \thetak_{\ell \sigma_{\ell}(a)}$. \\

For each $1 \leq \ell \leq \numgroups$, define the infeasible estimator 
\begin{align*}
\infeastheta_{\ell a} = \thetak_{\ell a} \quad \forall a \in [k^0_{\ell}] \quad \text{and} \quad \infeasc_i = \wh{c}_i(\infeastheta)
\end{align*}

That is, for each $1 \leq \ell \leq \numgroups$, we trim $k_{\ell} - k^0_{\ell}$ clusters from $\thetak$, leaving only those that solve $x^*_{\ell} = (\argmin_{x \in \clusterspace^k} \|\wh{\theta}^k(x) - \theta^0(c)\|^2)_{\ell}$ for some $\ell$. 
Then $(\infeastheta, \infeasgamma) \in \Theta^{k_0} \times \Gamma^{k_0}$ and $\infeastheta \convp \theta^0$ in the usual sense. 
Let $\qtilde$ be defined as above. 
To simplify notation, define $\modelk = (\thetak, \gammak)$, $\infeasmodel = (\infeastheta, \infeasgamma)$, $\modelknot = (\wh{\theta}^{k_0}, \wh{\gamma}^{k_0})$ and $\modeltrue = (\theta^0, \gamma^0)$. 
\begin{align*}
\qtilde(\infeasmodel) &= \qhat(\infeasmodel) + (\qtilde - \qhat)(\infeasmodel) \\
&= \qhat(\modelk) + (\qhat(\infeasmodel) - \qhat(\modelk)) + (\qtilde - \qhat)(\infeasmodel)\\
&= \qhat(\modelknot) + (\qhat(\modelk) - \qhat(\modelknot) +  (\qhat(\infeasmodel) - \qhat(\modelk)) + (\qtilde - \qhat)(\infeasmodel) \\
&\leq  \qtilde(\modelknot) + (\qhat - \qtilde)(\modelknot) + (\qhat(\infeasmodel) - \qhat(\modelk)) + (\qtilde - \qhat)(\infeasmodel) \\
&=  \qtilde(\modeltrue) + (\qtilde(\modelknot) - \qtilde(\modeltrue)) + (\qhat - \qtilde)(\modelknot) +  (\qhat(\infeasmodel) - \qhat(\modelk)) + (\qtilde - \qhat)(\infeasmodel)
\end{align*}

where the inequality follows because $k \geq k^0$. 
First consider 
\begin{equation*}
(\qtilde(\modelknot) - \qtilde(\modeltrue)) = \frac{1}{NT} \sum_{i, t} (x_{it}'(\theta^0(c_i^0) - \wh{\theta}^{k_0}(\wh{c}_i)))^2 = O_p(1/NT) + o_p(T^{-a})
\end{equation*}

because $(\wh{\theta}^{k_0}, \wh{\gamma}^{k_0})$ satisfies the conditions of lemma \ref{lemma:model:qk}. 
Similarly, the second term
\begin{equation*}
(\qhat(\modelknot) - \qtilde(\modelknot)) = \frac{2}{NT} \sum_{i, t} e_{it} x_{it}'(\theta^0(c_i^0) - \wh{\theta}^{k_0}(\wh{c}_i)) = O_p(1/NT) + o_p(T^{-a})
\end{equation*}

Since $\infeastheta \convp \theta^0$ and $\infeasc_i = \wh{c}_i(\infeastheta)$ for all $i$, the final term also satisfies the conditions of lemma \ref{lemma:model:qk}, so that
\begin{equation*}
(\qhat(\infeasmodel) - \qtilde(\infeasmodel)) = \frac{2}{NT} \sum_{i, t} e_{it} x_{it}'(\theta^0(c_i^0) - \infeastheta(\infeasc_i)) = o_p(1/\sqrt{NT}) + o_p(T^{-a})
\end{equation*}

To compare the sample risk of $\thetak$ and the infeasible $\infeastheta$, we note that by definition of $\thetak$, for every $i$ we have $\sum_t (y_{it} - \thetak(\wh{c}_i^k))^2 &\leq \sum_t (y_{it} - \infeastheta(\infeasc_i))^2$, that is
\begin{align} 
\sum_t e_{it} x_{it}'(\theta^0(\ctrue) - \thetak(\wh{c}_i^k)) &+ \frac{1}{NT} \sum_{i, t} (x_{it}'(\theta^0(\ctrue) - \thetak(\wh{c}_i^k)))^2 \leq \sum_t e_{it} x_{it}'(\theta^0(\ctrue) - \infeastheta(\infeasc_i) \nonumber \\
&+ \frac{1}{NT} \sum_{i, t} (x_{it}'(\theta^0(\ctrue) - \infeastheta(\infeasc))^2
\end{align}


==> blocked multiple regression - arxiv/table1_separation.tex <==
% Table generated by Excel2LaTeX from sheet 'ar'
\begin{table}[htbp]
  \centering
  \caption{Effect of Cluster Separation}
    \begin{tabular}{lllllllllllll}
          &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
          &       & \multicolumn{2}{c}{Coverage} &       & \multicolumn{2}{c}{Bootstrap Coverage} &       & \multicolumn{2}{c}{Param. MSE} &       & \multicolumn{2}{c}{Cluster Loss} \\
    \multicolumn{1}{c}{Angle ($\alpha$)} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} \\
\cmidrule{1-1}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}\cmidrule{12-13}    \multicolumn{1}{c}{1.57} &       & \multicolumn{1}{c}{0.90} & \multicolumn{1}{c}{0.89} &       & \multicolumn{1}{c}{0.88} & \multicolumn{1}{c}{0.87} &       & \multicolumn{1}{c}{0.047} & \multicolumn{1}{c}{0.053} &       & \multicolumn{1}{c}{0.044} & \multicolumn{1}{c}{0.050} \\
    \multicolumn{1}{c}{1.26} &       & \multicolumn{1}{c}{0.86} & \multicolumn{1}{c}{0.84} &       & \multicolumn{1}{c}{0.83} & \multicolumn{1}{c}{0.81} &       & \multicolumn{1}{c}{0.055} & \multicolumn{1}{c}{0.061} &       & \multicolumn{1}{c}{0.074} & \multicolumn{1}{c}{0.083} \\
    \multicolumn{1}{c}{0.94} &       & \multicolumn{1}{c}{0.75} & \multicolumn{1}{c}{0.72} &       & \multicolumn{1}{c}{0.73} & \multicolumn{1}{c}{0.69} &       & \multicolumn{1}{c}{0.059} & \multicolumn{1}{c}{0.067} &       & \multicolumn{1}{c}{0.13} & \multicolumn{1}{c}{0.14} \\
    \multicolumn{1}{c}{0.63} &       & \multicolumn{1}{c}{0.53} & \multicolumn{1}{c}{0.50} &       & \multicolumn{1}{c}{0.51} & \multicolumn{1}{c}{0.49} &       & \multicolumn{1}{c}{0.058} & \multicolumn{1}{c}{0.064} &       & \multicolumn{1}{c}{0.22} & \multicolumn{1}{c}{0.23} \\
    \multicolumn{1}{c}{0.31} &       & \multicolumn{1}{c}{0.25} & \multicolumn{1}{c}{0.25} &       & \multicolumn{1}{c}{0.24} & \multicolumn{1}{c}{0.24} &       & \multicolumn{1}{c}{0.052} & \multicolumn{1}{c}{0.059} &       & \multicolumn{1}{c}{0.37} & \multicolumn{1}{c}{0.38} \\
    \multicolumn{1}{c}{0.16} &       & \multicolumn{1}{c}{0.20} & \multicolumn{1}{c}{0.19} &       & \multicolumn{1}{c}{0.20} & \multicolumn{1}{c}{0.19} &       & \multicolumn{1}{c}{0.048} & \multicolumn{1}{c}{0.054} &       & \multicolumn{1}{c}{0.44} & \multicolumn{1}{c}{0.44} \\
    \midrule
    \multicolumn{13}{l}{\textit{Notes: N=150, T=10}} \\
    \end{tabular}%
  \label{table:separation}%
\end{table}%


==> blocked multiple regression - arxiv/table2_nt.tex <==
% Table generated by Excel2LaTeX from sheet 'means'
% Table generated by Excel2LaTeX from sheet 'hk'
\begin{table}[htbp]
  \centering
  \caption{Effect of Sample Size (N, T)}
   \begin{adjustbox}{width=1.1\columnwidth,center} 
    \begin{tabular}{r|cccccccccccccccccc}
    \multicolumn{1}{c}{} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{r}{} &       & \multicolumn{5}{c}{Param. MSE} &       & \multicolumn{5}{c}{Coverage (Analytical)} &       & \multicolumn{5}{c}{Cluster Loss} \\
\cmidrule{3-7}\cmidrule{9-13}\cmidrule{15-19}    \multicolumn{1}{l}{Errors} & T     & N=50  & 100   & 150   & 200   & 250   &       & 50    & 100   & 150   & 200   & 250   &       & 50    & 100   & 150   & 200   & 250 \\
    \midrule
          & 5     & 0.154 & 0.140 & 0.137 & 0.134 & 0.133 &       & 0.761 & 0.763 & 0.772 & 0.768 & 0.756 &       & 0.134 & 0.125 & 0.125 & 0.123 & 0.123 \\
    \multicolumn{1}{l|}{AR(1)} & 10    & 0.051 & 0.047 & 0.047 & 0.046 & 0.046 &       & 0.873 & 0.889 & 0.898 & 0.899 & 0.901 &       & 0.046 & 0.044 & 0.044 & 0.044 & 0.044 \\
          & 15    & 0.021 & 0.019 & 0.018 & 0.018 & 0.018 &       & 0.909 & 0.927 & 0.939 & 0.927 & 0.926 &       & 0.018 & 0.017 & 0.017 & 0.017 & 0.017 \\
          & 20    & 0.009 & 0.008 & 0.008 & 0.008 & 0.007 &       & 0.916 & 0.939 & 0.935 & 0.935 & 0.935 &       & 0.007 & 0.007 & 0.007 & 0.007 & 0.007 \\
          & 25    & 0.005 & 0.004 & 0.004 & 0.004 & 0.003 &       & 0.930 & 0.937 & 0.936 & 0.941 & 0.943 &       & 0.003 & 0.003 & 0.003 & 0.003 & 0.003 \\
    \multicolumn{1}{r}{} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
          & 5     & 0.160 & 0.146 & 0.144 & 0.143 & 0.140 &       & 0.718 & 0.748 & 0.738 & 0.738 & 0.736 &       & 0.137 & 0.130 & 0.130 & 0.130 & 0.128 \\
    \multicolumn{1}{l|}{HK} & 10    & 0.059 & 0.055 & 0.053 & 0.052 & 0.051 &       & 0.856 & 0.875 & 0.886 & 0.888 & 0.887 &       & 0.053 & 0.051 & 0.050 & 0.049 & 0.049 \\
          & 15    & 0.027 & 0.024 & 0.023 & 0.023 & 0.022 &       & 0.905 & 0.914 & 0.916 & 0.920 & 0.917 &       & 0.023 & 0.022 & 0.021 & 0.022 & 0.021 \\
          & 20    & 0.013 & 0.011 & 0.011 & 0.010 & 0.010 &       & 0.915 & 0.927 & 0.930 & 0.936 & 0.941 &       & 0.010 & 0.010 & 0.010 & 0.009 & 0.009 \\
          & 25    & 0.007 & 0.006 & 0.005 & 0.005 & 0.005 &       & 0.924 & 0.936 & 0.946 & 0.946 & 0.942 &       & 0.004 & 0.004 & 0.005 & 0.004 & 0.004 \\
    \bottomrule
    \end{tabular}%
    \end{adjustbox}
  \label{table:nt}%
\end{table}%


==> blocked multiple regression - arxiv/table3_clusters.tex <==
% Table generated by Excel2LaTeX from sheet 'ar'
\begin{table}[htbp]
  \centering
  \caption{Effect of Number of Clusters $(k_1, k_2)$}
   \begin{adjustbox}{width=1.1\columnwidth,center} 
    \begin{tabular}{lrrrrrrrrrrrrrr}
          &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{c}{\# Clusters} & \multicolumn{2}{c}{Coverage} &       & \multicolumn{2}{c}{Bootstrap Coverage} &       & \multicolumn{2}{c}{Param. MSE} &       & \multicolumn{2}{c}{Function MSE} &       & \multicolumn{2}{c}{Cluster Loss} \\
    \multicolumn{1}{c}{(k1, k2)} & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} \\
\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}\cmidrule{11-12}\cmidrule{14-15}    \multicolumn{1}{c}{(1, 2)} & \multicolumn{1}{c}{0.90} & \multicolumn{1}{c}{0.88} &       & \multicolumn{1}{c}{0.88} & \multicolumn{1}{c}{0.86} &       & \multicolumn{1}{c}{0.026} & \multicolumn{1}{c}{0.030} &       & \multicolumn{1}{c}{0.026} & \multicolumn{1}{c}{0.094} &       & \multicolumn{1}{c}{0.035} & \multicolumn{1}{c}{0.040} \\
    \multicolumn{1}{c}{(2, 2)} & \multicolumn{1}{c}{0.86} & \multicolumn{1}{c}{0.83} &       & \multicolumn{1}{c}{0.83} & \multicolumn{1}{c}{0.81} &       & \multicolumn{1}{c}{0.054} & \multicolumn{1}{c}{0.063} &       & \multicolumn{1}{c}{0.054} & \multicolumn{1}{c}{0.184} &       & \multicolumn{1}{c}{0.074} & \multicolumn{1}{c}{0.085} \\
    \multicolumn{1}{c}{(2, 3)} & \multicolumn{1}{c}{0.84} & \multicolumn{1}{c}{0.81} &       & \multicolumn{1}{c}{0.82} & \multicolumn{1}{c}{0.79} &       & \multicolumn{1}{c}{0.070} & \multicolumn{1}{c}{0.078} &       & \multicolumn{1}{c}{0.070} & \multicolumn{1}{c}{0.218} &       & \multicolumn{1}{c}{0.090} & \multicolumn{1}{c}{0.100} \\
    \multicolumn{1}{c}{(3, 3)} & \multicolumn{1}{c}{0.81} & \multicolumn{1}{c}{0.78} &       & \multicolumn{1}{c}{0.80} & \multicolumn{1}{c}{0.76} &       & \multicolumn{1}{c}{0.085} & \multicolumn{1}{c}{0.095} &       & \multicolumn{1}{c}{0.085} & \multicolumn{1}{c}{0.258} &       & \multicolumn{1}{c}{0.106} & \multicolumn{1}{c}{0.119} \\
    \multicolumn{1}{c}{(3, 4)} & \multicolumn{1}{c}{0.80} & \multicolumn{1}{c}{0.76} &       & \multicolumn{1}{c}{0.78} & \multicolumn{1}{c}{0.74} &       & \multicolumn{1}{c}{0.099} & \multicolumn{1}{c}{0.109} &       & \multicolumn{1}{c}{0.099} & \multicolumn{1}{c}{0.281} &       & \multicolumn{1}{c}{0.118} & \multicolumn{1}{c}{0.131} \\
    \multicolumn{1}{c}{(4, 4)} & \multicolumn{1}{c}{0.77} & \multicolumn{1}{c}{0.73} &       & \multicolumn{1}{c}{0.76} & \multicolumn{1}{c}{0.72} &       & \multicolumn{1}{c}{0.114} & \multicolumn{1}{c}{0.123} &       & \multicolumn{1}{c}{0.114} & \multicolumn{1}{c}{0.306} &       & \multicolumn{1}{c}{0.132} & \multicolumn{1}{c}{0.143} \\
    \midrule
    \multicolumn{15}{l}{\textit{Notes: N=150, T=10}} \\
    \end{tabular}%
    \end{adjustbox}
  \label{table:clusters}%
\end{table}%


==> blocked multiple regression - arxiv/table4_misspec.tex <==
% Table generated by Excel2LaTeX from sheet 'ar'
\begin{table}[htbp]
  \centering
  \caption{Effect of Misspecified Blocking of Covariates - Estimation with $B^0=1$ and $B=2$}
    \begin{tabular}{lrrrrrrr}
          &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{c}{Errors} & \multicolumn{1}{c}{\# Clusters} &       & \multicolumn{2}{c}{Param. MSE} &       & \multicolumn{2}{c}{Function MSE} \\
          & \multicolumn{1}{c}{(k1, k2)} &       & \multicolumn{1}{c}{B=1} & \multicolumn{1}{c}{B=2} &       & \multicolumn{1}{c}{B=1} & \multicolumn{1}{c}{B=2} \\
\cmidrule{2-2}\cmidrule{4-5}\cmidrule{7-8}          & \multicolumn{1}{c}{(1, 2)} &       & 0.027 & 0.026 &       & 0.077 & \multicolumn{1}{c}{0.026} \\
          & \multicolumn{1}{c}{(2, 2)} &       & 0.058 & 0.054 &       & 0.157 & \multicolumn{1}{c}{0.054} \\
    \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{(2, 3)} &       & 0.079 & 0.070 &       & 0.206 & \multicolumn{1}{c}{0.070} \\
          & \multicolumn{1}{c}{(3, 3)} &       & 0.108 & 0.085 &       & 0.273 & \multicolumn{1}{c}{0.085} \\
          & \multicolumn{1}{c}{(3, 4)} &       & 0.137 & 0.099 &       & 0.334 & \multicolumn{1}{c}{0.099} \\
          & \multicolumn{1}{c}{(4, 4)} &       & 0.163 & 0.114 &       & 0.383 & \multicolumn{1}{c}{0.114} \\
          &       &       &       &       &       &       &  \\
          &       &       & \multicolumn{1}{c}{B=1} & \multicolumn{1}{c}{B=2} &       & \multicolumn{1}{c}{B=1} & \multicolumn{1}{c}{B=2} \\
\cmidrule{2-2}\cmidrule{4-5}\cmidrule{7-8}          & \multicolumn{1}{c}{(1, 2)} &       & 0.031 & \multicolumn{1}{c}{0.030} &       & 0.097 & \multicolumn{1}{c}{0.094} \\
          & \multicolumn{1}{c}{(2, 2)} &       & 0.068 & \multicolumn{1}{c}{0.063} &       & 0.200 & \multicolumn{1}{c}{0.184} \\
    \multicolumn{1}{c}{HK} & \multicolumn{1}{c}{(2, 3)} &       & 0.090 & \multicolumn{1}{c}{0.078} &       & 0.252 & \multicolumn{1}{c}{0.218} \\
          & \multicolumn{1}{c}{(3, 3)} &       & 0.122 & \multicolumn{1}{c}{0.095} &       & 0.335 & \multicolumn{1}{c}{0.258} \\
          & \multicolumn{1}{c}{(3, 4)} &       & 0.149 & \multicolumn{1}{c}{0.109} &       & 0.393 & \multicolumn{1}{c}{0.281} \\
          & \multicolumn{1}{c}{(4, 4)} &       & 0.174 & \multicolumn{1}{c}{0.123} &       & 0.441 & \multicolumn{1}{c}{0.306} \\
    \midrule
    \multicolumn{8}{l}{\textit{Notes: N=150, T=10}} \\
    \end{tabular}%
  \label{table:misspec}%
\end{table}%


==> blocked multiple regression - arxiv/table5_imbalance.tex <==
% Table generated by Excel2LaTeX from sheet 'ar'
\begin{table}[htbp]
  \centering
  \caption{Effect of Dimension Imbalance}
   \begin{adjustbox}{width=1\columnwidth,center} 
    \begin{tabular}{lrrrrrrrrrrrrrr}
          &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{1}{c}{dim} & \multicolumn{2}{c}{Coverage-large} &       & \multicolumn{2}{c}{Coverage-small} &       & \multicolumn{2}{c}{Cluster loss-small} &       & \multicolumn{2}{c}{Cluster loss-large} &       & \multicolumn{2}{c}{Param. MSE} \\
    \multicolumn{1}{c}{(m, p-m)} & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} &       & \multicolumn{1}{c}{AR(1)} & \multicolumn{1}{c}{HK} \\
\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}\cmidrule{11-12}\cmidrule{14-15}    \multicolumn{1}{c}{(1, 11)} & \multicolumn{1}{c}{0.921} & \multicolumn{1}{c}{0.918} &       & \multicolumn{1}{c}{0.599} & \multicolumn{1}{c}{0.538} &       & \multicolumn{1}{c}{0.156} & \multicolumn{1}{c}{0.170} &       & \multicolumn{1}{c}{0.000} & \multicolumn{1}{c}{0.000} &       & \multicolumn{1}{c}{0.009} & \multicolumn{1}{c}{0.009} \\
    \multicolumn{1}{c}{(2, 10)} & \multicolumn{1}{c}{0.930} & \multicolumn{1}{c}{0.931} &       & \multicolumn{1}{c}{0.841} & \multicolumn{1}{c}{0.840} &       & \multicolumn{1}{c}{0.069} & \multicolumn{1}{c}{0.060} &       & \multicolumn{1}{c}{0.001} & \multicolumn{1}{c}{0.001} &       & \multicolumn{1}{c}{0.008} & \multicolumn{1}{c}{0.007} \\
    \multicolumn{1}{c}{(3, 9)} & \multicolumn{1}{c}{0.932} & \multicolumn{1}{c}{0.931} &       & \multicolumn{1}{c}{0.917} & \multicolumn{1}{c}{0.910} &       & \multicolumn{1}{c}{0.029} & \multicolumn{1}{c}{0.028} &       & \multicolumn{1}{c}{0.001} & \multicolumn{1}{c}{0.001} &       & \multicolumn{1}{c}{0.006} & \multicolumn{1}{c}{0.006} \\
    \multicolumn{1}{c}{(4, 8)} & \multicolumn{1}{c}{0.935} & \multicolumn{1}{c}{0.930} &       & \multicolumn{1}{c}{0.922} & \multicolumn{1}{c}{0.916} &       & \multicolumn{1}{c}{0.016} & \multicolumn{1}{c}{0.019} &       & \multicolumn{1}{c}{0.001} & \multicolumn{1}{c}{0.001} &       & \multicolumn{1}{c}{0.005} & \multicolumn{1}{c}{0.005} \\
    \multicolumn{1}{c}{(5, 7)} & \multicolumn{1}{c}{0.931} & \multicolumn{1}{c}{0.934} &       & \multicolumn{1}{c}{0.927} & \multicolumn{1}{c}{0.934} &       & \multicolumn{1}{c}{0.006} & \multicolumn{1}{c}{0.007} &       & \multicolumn{1}{c}{0.003} & \multicolumn{1}{c}{0.002} &       & \multicolumn{1}{c}{0.005} & \multicolumn{1}{c}{0.005} \\
    \multicolumn{1}{c}{(6, 6)} & \multicolumn{1}{c}{0.936} & \multicolumn{1}{c}{0.938} &       & \multicolumn{1}{c}{0.939} & \multicolumn{1}{c}{0.935} &       & \multicolumn{1}{c}{0.003} & \multicolumn{1}{c}{0.003} &       & \multicolumn{1}{c}{0.004} & \multicolumn{1}{c}{0.004} &       & \multicolumn{1}{c}{0.004} & \multicolumn{1}{c}{0.004} \\
    \midrule
    \textit{Notes: N=150, T=10} &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \end{tabular}%
    \end{adjustbox}
  \label{table:imbalance}%
\end{table}%


==> blocked multiple regression - arxiv/table6_dimension.tex <==
% Table generated by Excel2LaTeX from sheet 'means'
\begin{table}[htbp]
  \centering
  \caption{Effect of Growing Model Dimension}
    \begin{tabular}{lrrrrrrrrrrrrrr}
          &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
\cmidrule{1-12}    \multicolumn{1}{c}{dim (p)} & \multicolumn{2}{c}{Coverage} &       & \multicolumn{2}{c}{Param. MSE} &       & \multicolumn{2}{c}{Function MSE} &       & \multicolumn{2}{c}{Cluster Loss} &       &       &  \\
    \multicolumn{1}{c}{Error} & \multicolumn{1}{c}{indep} & \multicolumn{1}{c}{AR(1)} &       & \multicolumn{1}{c}{indep} & \multicolumn{1}{c}{AR(1)} &       & \multicolumn{1}{c}{indep} & \multicolumn{1}{c}{AR(1)} &       & \multicolumn{1}{c}{indep} & \multicolumn{1}{c}{AR(1)} &       &       &  \\
\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}\cmidrule{11-12}    \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0.93} & \multicolumn{1}{c}{0.92} &       & \multicolumn{1}{c}{0.046} & \multicolumn{1}{c}{0.078} &       & \multicolumn{1}{c}{0.023} & \multicolumn{1}{c}{0.065} &       & \multicolumn{1}{c}{0.011} & \multicolumn{1}{c}{0.019} &       &       &  \\
    \multicolumn{1}{c}{2} & \multicolumn{1}{c}{0.94} & \multicolumn{1}{c}{0.91} &       & \multicolumn{1}{c}{0.047} & \multicolumn{1}{c}{0.060} &       & \multicolumn{1}{c}{0.045} & \multicolumn{1}{c}{0.077} &       & \multicolumn{1}{c}{0.012} & \multicolumn{1}{c}{0.015} &       &       &  \\
    \multicolumn{1}{c}{3} & \multicolumn{1}{c}{0.92} & \multicolumn{1}{c}{0.93} &       & \multicolumn{1}{c}{0.051} & \multicolumn{1}{c}{0.059} &       & \multicolumn{1}{c}{0.067} & \multicolumn{1}{c}{0.095} &       & \multicolumn{1}{c}{0.012} & \multicolumn{1}{c}{0.014} &       &       &  \\
    \multicolumn{1}{c}{4} & \multicolumn{1}{c}{0.91} & \multicolumn{1}{c}{0.92} &       & \multicolumn{1}{c}{0.058} & \multicolumn{1}{c}{0.063} &       & \multicolumn{1}{c}{0.098} & \multicolumn{1}{c}{0.122} &       & \multicolumn{1}{c}{0.014} & \multicolumn{1}{c}{0.015} &       &       &  \\
    \multicolumn{1}{c}{5} & \multicolumn{1}{c}{0.92} & \multicolumn{1}{c}{0.90} &       & \multicolumn{1}{c}{0.064} & \multicolumn{1}{c}{0.068} &       & \multicolumn{1}{c}{0.127} & \multicolumn{1}{c}{0.150} &       & \multicolumn{1}{c}{0.015} & \multicolumn{1}{c}{0.016} &       &       &  \\
\cmidrule{1-12}    \multicolumn{15}{l}{\textit{Notes: N=150, T=10}} \\
    \end{tabular}%
  \label{table:dimension}%
\end{table}%


==> blocked multiple regression - arxiv/table_computational_experiments.tex <==
% Table generated by Excel2LaTeX from sheet 'exp1'
\begin{table}[htbp]
  \centering
    \caption{Number of Initializations for 0.1\% Rel. Error}
    \begin{tabular}{rrrrrrrrr}
          &       &       &       &       &       &       &       &  \\
    \midrule
          &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{c}{(N, T)} &       & \multicolumn{1}{c}{$s_{\theta}$} & \multicolumn{1}{c}{$s_q$} &       & \multicolumn{1}{c}{Angle} &       & \multicolumn{1}{c}{$s_{\theta}$} & \multicolumn{1}{c}{$s_q$} \\
\cmidrule{1-1}\cmidrule{3-4}\cmidrule{6-6}\cmidrule{8-9}    \multicolumn{1}{c}{(20, 10)} &       & \multicolumn{1}{c}{84} & \multicolumn{1}{c}{9} &       & \multicolumn{1}{c}{1} &       & \multicolumn{1}{c}{14} & \multicolumn{1}{c}{0} \\
    \multicolumn{1}{c}{(50, 10)} &       & \multicolumn{1}{c}{65} & \multicolumn{1}{c}{1} &       & \multicolumn{1}{c}{0.8} &       & \multicolumn{1}{c}{98} & \multicolumn{1}{c}{0} \\
    \multicolumn{1}{c}{(100, 10)} &       & \multicolumn{1}{c}{28} & \multicolumn{1}{c}{0} &       & \multicolumn{1}{c}{0.6} &       & \multicolumn{1}{c}{56} & \multicolumn{1}{c}{0} \\
    \multicolumn{1}{c}{(150, 10)} &       & \multicolumn{1}{c}{9} & \multicolumn{1}{c}{0} &       & \multicolumn{1}{c}{0.4} &       & \multicolumn{1}{c}{109} & \multicolumn{1}{c}{2} \\
    \multicolumn{1}{c}{(250, 10)} &       & \multicolumn{1}{c}{7} & \multicolumn{1}{c}{0} &       & \multicolumn{1}{c}{0.2} &       & \multicolumn{1}{c}{139} & \multicolumn{1}{c}{4} \\
          &       &       &       &       & \multicolumn{1}{c}{0.1} &       & \multicolumn{1}{c}{157} & \multicolumn{1}{c}{5} \\
          &       &       &       &       &       &       &       &  \\
    \multicolumn{1}{c}{(N, T)} &       & \multicolumn{1}{c}{$s_{\theta}$} & \multicolumn{1}{c}{$s_q$} &       & \multicolumn{1}{c}{K} &       & \multicolumn{1}{c}{$s_{\theta}$} & \multicolumn{1}{c}{$s_q$} \\
\cmidrule{1-1}\cmidrule{3-4}\cmidrule{6-6}\cmidrule{8-9}    \multicolumn{1}{c}{(50, 5)} &       & \multicolumn{1}{c}{163} & \multicolumn{1}{c}{10} &       & \multicolumn{1}{c}{3} &       & \multicolumn{1}{c}{14} & \multicolumn{1}{c}{1} \\
    \multicolumn{1}{c}{(50, 15)} &       & \multicolumn{1}{c}{17} & \multicolumn{1}{c}{0} &       & \multicolumn{1}{c}{4} &       & \multicolumn{1}{c}{48} & \multicolumn{1}{c}{0} \\
    \multicolumn{1}{c}{(50, 20)} &       & \multicolumn{1}{c}{9} & \multicolumn{1}{c}{1} &       & \multicolumn{1}{c}{5} &       & \multicolumn{1}{c}{153} & \multicolumn{1}{c}{1} \\
    \multicolumn{1}{c}{(50, 25)} &       & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{0} &       & \multicolumn{1}{c}{6} &       & \multicolumn{1}{c}{130} & \multicolumn{1}{c}{4} \\
          &       &       &       &       & \multicolumn{1}{c}{7} &       & \multicolumn{1}{c}{163} & \multicolumn{1}{c}{4} \\
    \midrule
    \multicolumn{9}{r}{} \\
    \end{tabular}%
  \label{table:computation:relative_error}%
\end{table}%


==> old_text.tex <==
%%% OLD COMPUTATIONAL SECTION ON FULL AND PARTIAL UPDATES

The current implementation of our algorithm performs coordinate ascent on $\theta$ by updating one matrix $\theta_{\ell}$ at a time, as described below in the partial update case. 
An alternative is to solve the full update for all of the blocks $1 \leq \ell \leq \numgroups$ simultaneously, though this is potentially much slower computationally. 
Both alternatives are described below. \\

\textbf{Full Parameter Update} \\

In step (3) of our algorithm,we can perform a full parameter update, setting $\theta^{t + 1} = \argmin_{\theta \in \Theta} \samplerisk(\theta, \gamma^{t + 1})$
To describe the full update, we define $\indsubcluster = \{i: \gamma_{\ell}(i) = a\}$, where $a \in [k_{\ell}]$.
Recall that $\theta = \{\theta_1, \dots, \theta_{\ell}\}$, the collection of parameters for each block, and we can view $\theta_{\ell}$ as a matrix $\theta_{\ell} \in \mathbb{R}^{d_{\ell} \times k_{\ell}}$ that collects the parameters for each cluster in the block in the columns of $\theta_{\ell}$.
Then setting $\nabla_{\thetasuba} \samplerisk(\theta, \gamma) = 0$ gives

\begin{align*}
\sum_{i \in \indsubcluster} y_i \xell &= \sum_{\ellt} \sum_{i \in \indsubcluster} \sum_{t} \xell \xellp \theta_{\ellt}(c_i) = \sum_{\ellt} \sum_{i \in \indsubcluster} \sum_{t} \sum_{b = 1}^{k_{\ellt}} \mathds{1}(\cilt = b) \xell \xellp \theta_{\ellt}(c_i) \\
&= \sum_{\ellt} \sum_{b=1}^{k_{\ellt}} \left (\sum_{t, i \in \indsubcluster} \mathds{1}(\cilt = b) \xell \xellp \right ) \theta_{\ellt b} \equiv \sum_{\ellt} \sum_{b=1}^{k_{\ellt}} M_{\ell a, \ellt b} \theta_{\ellt b}
\end{align*}

Define $\vect(\theta) = (\vect(\theta_1), \dots, \vect(\theta_{\numgroups}))$ and $v_{\ell a} = \sum_{i \in \indsubcluster} y_i \xell$, then $\argmin_{\theta \in \Theta} \samplerisk(\theta, \gamma)$ is given by the solution to 

\begin{equation} \label{full_update}
v = M \vect(\theta)
\end{equation}

Here indices of the form $M_{\ell a, \ellt b}$ are block indices, e.g. giving the indices corresponding to the $a^{th}$ cluster of the $\ell^{th}$ block. 
Letting $d_{max} \equiv \max_{\ell} d_{\ell}$, then the time complexity of the algorithm that solves the equation in \ref{full_update} is $\bigo \left (n d_{max}^2 + \left ( \sum_{\ell} k_{\ell} d_{\ell} \right )^3 \right)$ (assuming cubic time to solve the linear equation).
Note that many of the $M_{\ell a, \ellt b }$ sub-matrices may be zero, so it's possible that a sparse solver may do better. \\

\textbf{Partial Parameter Update} \\

Another option is to update $\theta = (\theta_1, \dots \theta_{\numgroups})$ sequentially, e.g. letting 

\[
\theta_{\ell}^{t + 1} = \argmin_{\theta \in \Theta_{\ell}} L_{N, T}(\theta^{t + 1}_{1:\ell-1}, \theta_{\ell}, \theta^t_{\ell + 1:\numgroups}, \gamma^{t + 1})
\]

for each $1 \leq \ell \leq \numgroups$.
By additive separability of $\samplerisk$ in $\theta_{\ell a}$ over $a \in [k_{\ell}]$, this is equivalent to solving 

\[
\argmin_{\thetasuba \in \mathbb{R}^{d_{\ell}}} \sum_{t, i \in \indsubcluster} (y_{it} - \xell' \thetasuba - f(x_{it}, \theta_{- \ell}))^2
\]

This can be solved by computing the panel regression of $y_{it} - f(x_{it}, \theta_{- \ell})$ on $\xell$ over the subset $\indsubcluster$.
Repeating this for each $1 \leq \ell \leq \numgroups$ and $a \in [k_{\ell}]$ has time complexity $\bigo \left (n d_{max}^2 + \sum_{\ell} k_{\ell} d_{\ell}^3 \right )$, potentially significantly better than (the naive implementation of) the full update above. \\

\textbf{Initialization} \\

In our simulations, we let initialize cluster assignments by setting $\cil^1 \sim \{1, \dots, k_{\ell}\}$ uniformly, and independently over $i, \ell$.
We take $\thetasuba \sim N(0, 1)$, independently over $\ell, a$. 
There are some other potential initialization schemes that may lead to quicker convergence in practice. 


%%% Previous ``throw away extra clusters'' approach to proving rates / consistency for the over-specified estimator

\subsection{Old Approaches [Not Currently Used]}

% WORKING PROOF
In what follows, we outline an attack on (i). 
We start by describing the sense in which $\thetak$ is consistent for $\theta^0$ when $k \geq k^0$. 
With $\qtilde$ defined as in our consistency proof in equation \ref{equation:qtilde_def}, we have 
\begin{align*}
\qtilde(\thetak, \gammak) &= \wh{Q}(\thetak, \gammak) + [\qtilde(\thetak, \gammak) - \wh{Q}(\thetak, \gammak)] \leq \wh{Q}(\thetak, \gammak) + \sup_{\theta \in \Theta^k, \gamma \in \Gamma^k} \left [(\qtilde - \wh{Q})(\thetak, \gammak) \right ]\\
&= \wh{Q}(\thetak, \gammak) + o_P(1) \leq \wh{Q}(\theta^0, \gamma^0) + o_P(1) = \qtilde(\theta^0, \gamma^0) + o_P(1) 
\end{align*}

% note - can make cmpt assumption more explicit for k not k^0
The third expression  
Note that we now sup over $(\Theta^k, \Gamma^k)$, but the second inequality still holds as long as $\text{Im}(\theta^k \circ \gamma^k)$ is compact.  
The second inequality still holds because $k \geq k^0 \implies$ $(\theta^0, \gamma^0)$ is in the parameter space of the misspecified estimator.\footnote{Specifically, there exist $\theta^k \in \Theta^k$ and $\gamma^k \in \Gamma^k$ such that the $N \times p$ matrix with i^{th} row $\theta^0(\gamma^0(i)) = \theta^k(\gamma^k(i))$ for all $i \in [N]$}
This shows that $0 \leq \qtilde(\thetak, \gammak) - \qtilde(\theta^0, \gamma^0) \leq o_P(1)$. 
Then our proof of part (ii) of the lemma shows
\begin{align*}
o_p(1) &\geq \qtilde(\thetak, \gammak) - \qtilde(\theta^0, \gamma^0) = \frac{1}{NT}\sum_{i, t} (x_{it}'(\theta^0(c_i^0) - \wh{\theta}^k(\cest^k))^2 \\
&\geq \delta \sum_{c' \in \mathcal{C}^{k_0}} \min_{x \in \mathcal{C}^k} \|\wh{\theta}^k(x) - \theta^0(c')\|^2 - o_p(1) \\
&\implies \min_{x \in \mathcal{C}^k} \|\wh{\theta}^k(x) - \theta^0(c)\|^2 = o_p(1) \quad \forall c \in \clusterspace^{k_0}
\end{align*}

using compactness in the second inequality. 
Since the square norm above is additively separable in the norms of each block of the covariate vector, for any $c, c' \in \clusterspace^{k_0}$ with $c_{\ell} = c'_{\ell}$, we must have $(\argmin_{x \in \clusterspace^k} \|\wh{\theta}^k(x) - \theta^0(c)\|^2)_{\ell} = (\argmin_{x \in \clusterspace^k} \|\wh{\theta}^k(x) - \theta^0(c')\|^2)_{\ell}$. 
This shows that setting $\sigma_{\ell}(a) = (\argmin_{x \in \clusterspace^k} \|\wh{\theta}^k(x) - \theta^0(c)\|^2)_{\ell}$ for any $c \in \clusterspace^{k_0}$ with $c_{\ell} = a$ is well-defined. 
As in the well-specified case, this relationship is 1-1 w.h.p. as $N, T \to \infty$ by well-separation of the true clusters in assumption \ref{consistency:separation}, so we relabel $\thetak_{\ell a} \equiv \thetak_{\ell \sigma_{\ell}(a)}$. \\

For each $1 \leq \ell \leq \numgroups$, define the infeasible estimator 
\begin{align*}
\infeastheta_{\ell a} = \thetak_{\ell a} \quad \forall a \in [k^0_{\ell}] \quad \text{and} \quad \infeasc_i = \wh{c}_i(\infeastheta)
\end{align*}

That is, for each $1 \leq \ell \leq \numgroups$, we trim $k_{\ell} - k^0_{\ell}$ clusters from $\thetak$, leaving only those that solve $x^*_{\ell} = (\argmin_{x \in \clusterspace^k} \|\wh{\theta}^k(x) - \theta^0(c)\|^2)_{\ell}$ for some $\ell$. 
Then $(\infeastheta, \infeasgamma) \in \Theta^{k_0} \times \Gamma^{k_0}$ and $\infeastheta \convp \theta^0$ in the usual sense. 
Let $\qtilde$ be defined as above. 
To simplify notation, define $\modelk = (\thetak, \gammak)$, $\infeasmodel = (\infeastheta, \infeasgamma)$, $\modelknot = (\wh{\theta}^{k_0}, \wh{\gamma}^{k_0})$ and $\modeltrue = (\theta^0, \gamma^0)$. 
\begin{align*}
\qtilde(\infeasmodel) &= \qhat(\infeasmodel) + (\qtilde - \qhat)(\infeasmodel) \\
&= \qhat(\modelk) + (\qhat(\infeasmodel) - \qhat(\modelk)) + (\qtilde - \qhat)(\infeasmodel)\\
&= \qhat(\modelknot) + (\qhat(\modelk) - \qhat(\modelknot) +  (\qhat(\infeasmodel) - \qhat(\modelk)) + (\qtilde - \qhat)(\infeasmodel) \\
&\leq  \qtilde(\modelknot) + (\qhat - \qtilde)(\modelknot) + (\qhat(\infeasmodel) - \qhat(\modelk)) + (\qtilde - \qhat)(\infeasmodel) \\
&=  \qtilde(\modeltrue) + (\qtilde(\modelknot) - \qtilde(\modeltrue)) + (\qhat - \qtilde)(\modelknot) +  (\qhat(\infeasmodel) - \qhat(\modelk)) + (\qtilde - \qhat)(\infeasmodel)
\end{align*}

where the inequality follows because $k \geq k^0$. 
First consider 
\begin{equation*}
(\qtilde(\modelknot) - \qtilde(\modeltrue)) = \frac{1}{NT} \sum_{i, t} (x_{it}'(\theta^0(c_i^0) - \wh{\theta}^{k_0}(\wh{c}_i)))^2 = O_p(1/NT) + o_p(T^{-a})
\end{equation*}

because $(\wh{\theta}^{k_0}, \wh{\gamma}^{k_0})$ satisfies the conditions of lemma \ref{lemma:model:qk}. 
Similarly, the second term
\begin{equation*}
(\qhat(\modelknot) - \qtilde(\modelknot)) = \frac{2}{NT} \sum_{i, t} e_{it} x_{it}'(\theta^0(c_i^0) - \wh{\theta}^{k_0}(\wh{c}_i)) = O_p(1/NT) + o_p(T^{-a})
\end{equation*}

Since $\infeastheta \convp \theta^0$ and $\infeasc_i = \wh{c}_i(\infeastheta)$ for all $i$, the final term also satisfies the conditions of lemma \ref{lemma:model:qk}, so that
\begin{equation*}
(\qhat(\infeasmodel) - \qtilde(\infeasmodel)) = \frac{2}{NT} \sum_{i, t} e_{it} x_{it}'(\theta^0(c_i^0) - \infeastheta(\infeasc_i)) = o_p(1/\sqrt{NT}) + o_p(T^{-a})
\end{equation*}

To compare the sample risk of $\thetak$ and the infeasible $\infeastheta$, we note that by definition of $\thetak$, for every $i$ we have $\sum_t (y_{it} - \thetak(\wh{c}_i^k))^2 &\leq \sum_t (y_{it} - \infeastheta(\infeasc_i))^2$, that is
\begin{align} 
\sum_t e_{it} x_{it}'(\theta^0(\ctrue) - \thetak(\wh{c}_i^k)) &+ \frac{1}{NT} \sum_{i, t} (x_{it}'(\theta^0(\ctrue) - \thetak(\wh{c}_i^k)))^2 \leq \sum_t e_{it} x_{it}'(\theta^0(\ctrue) - \infeastheta(\infeasc_i) \nonumber \\
&+ \frac{1}{NT} \sum_{i, t} (x_{it}'(\theta^0(\ctrue) - \infeastheta(\infeasc))^2
\end{align}

